Maximizing the electromomentum coupling in piezoelectric laminates

Asymmetric piezoelectric composites exhibit coupling between their macroscopic linear momentum and electric field, a coupling that does not appear at the microscopic scale. This electromomentum coupling constitutes an additional knob to tailor the dynamic response of the medium, analogously to the Willis coupling in elastic composites. Here, we employ topology- and free material optimization approaches to maximize the electromomentum coupling of periodic piezoelectric laminates in the low frequency, long-wavelength limit. We find that the coupling can be enhanced by orders of magnitude, depending on the degrees of freedom in the optimization process. The optimal compositions that we find provide guidelines for the design of metamaterials with maximum electromomentum coupling, paving the way for their integration in wave control applications.

==> Governing.tex <==
The governing equations of a piezoelectric medium are

\begin{equation}
\begin{aligned} & \div\stresst+\forcev=\dot{\momentumv},\\
 & \div\elecdispv=\charge,\\
 & \curl\elecfldv=\boldsymbol{0},
\end{aligned}
\end{equation}
where $\forcev$ is the body force density, $\stresst$ is the Cauchy
stress, $\momentumv$ is the linear momentum, $\elecdispv$ is the
electric displacement, $\charge$ is the charge density and $\elecfldv$
is the electric field. Note that $\curl\elecfldv=\boldsymbol{0}$
is identically satisfied by setting $\elecfldv=-\grad\elecpot$, where
$\elecpot$ is referred to as the electric potential.

The constitutive relations of the medium are
\begin{equation}
\left(\begin{array}{c}
\stresst\\
\elecdispv\\
\momentumv
\end{array}\right)=\left(\begin{array}{ccc}
\stiffnesst & \trans{\B} & 0\\
\B & -\A & 0\\
0 & 0 & \density
\end{array}\right)\left(\begin{array}{c}
\grad\dispv-\strainsot\\
\grad\elecpot\\
\dot{\dispv}
\end{array}\right),
\end{equation}
 where $\dispv$ is the displacement field and $\strainsot$ is the
inelastic strain. These properties are function of the position $\location$
when the medium is made of different piezoelectric materials. Assuming
time dependency in the form of $\mathrm{e}^{-i\angvel t}$ means that
time derivatives can be replaced by multiplication by $-i\angvel$.
Note that we take the real part or the imaginary part of the field
as our physical solution. \\
The one dimensional governing equation can be written as 
\begin{equation}
\begin{aligned} & \derivative{\stress}+\force=-i\angvel\momentum,\\
 & \derivative{\elecdisp}=\charge,
\end{aligned}
\label{eq:PiezoGov}
\end{equation}
and the constitutive relations are 
\begin{equation}
\left(\begin{array}{c}
\stress\\
\elecdisp\\
\momentum
\end{array}\right)=\left(\begin{array}{ccc}
\stiffness & \trans{\Bb} & 0\\
\Bb & -\Aa & 0\\
0 & 0 & \density
\end{array}\right)\left(\begin{array}{c}
\derivative{\disp}-\strainso\\
\derivative{\elecpot}\\
-i\angvel\disp
\end{array}\right).\label{eq:constPiezo}
\end{equation}
Homogenization shows that the effective constitutive relations have
a generalized Willis structure in the form
\begin{equation}
\left(\begin{array}{c}
\effective{\stresst}\\
\effective{\elecdispv}\\
\effective{\momentumv}
\end{array}\right)=\left(\begin{array}{ccc}
\effectiveprop{\stiffnesst} & \dag{\effectiveprop{\B}} & \effectiveprop{\couplingt}\\
\effectiveprop{\B} & -\effectiveprop{\A} & \effectiveprop{\couplingelet}\\
\dag{\effectiveprop{\couplingt}} & \dag{\effectiveprop{\couplingelet}} & \effectiveprop{\densityt}
\end{array}\right)\left(\begin{array}{c}
\effective{\grad\dispv}-\effective{\strainsot}\\
\effective{\grad\elecpot}\\
\effective{\dot{\dispv}}
\end{array}\right),\label{eq:GenWillis}
\end{equation}
where $\effective{\circ}$ denotes an effective field and $\effectiveprop{\left(\circ\right)}$
denotes an effective property. Our goal is to develop a method for
calculating the unique effective properties in a periodic medium.
To this end, we will employ a plane wave expansion approach, as we
develop in the next section.

==> Introduction.tex <==
Composites are modeled by macro-coupling parameters between the physical fields. 
Homogenization shows that by carefully designing a composite, supernatural properties can be achieved that cannot be found in its constituents.
Such materials are known as metamaterials.
Since the invention of artificial materials with exotic properties about a decades ago, considerable work has gone into the study of metamaterials. 
Metamaterials were developed in optics, acoustics and mechanics for various objectives \cite{craster2012acoustic, christensen2015vibrant, babaee20133d, padilla2006negative}. 
A principal objective of metamaterials is to manipulate the wave propagation \cite{banerjee2011introduction, parnell2013antiplane, celli2015manipulating}. 
A recent extraordinary property that has been discovered is a coupling between the macroscopic momentum and strain, termed Willis coupling \cite{willis1981variational, willis1985nonlocal, willis1997dynamics}. 
Since mechanical waves are governed by the balance of momentum, Willis coupling offers a designable degree of freedom to obtain control over waves. 
The theory of Willis gained interest and is still investigated by Willis \cite{willis2019statics} and others \cite{meng2018dynamic, muhlestein2016reciprocity, liu2019willis, chen2020active, norris2012analytical}.
These theoretical studies are supported by experiments that showed the immense potential of the Willis coupling in various applications \cite{chen2020active, su2018retrieval}. 
Hence, the demand for integrating, investigating and analysing structural optimization techniques and the theory of Willis has risen.
Recently, researchers engaged in maximizing the Willis coupling \cite{quan2018maximum, melnikov2019acoustic, muhlestein2019optimization}. 
Results show that optimal designs exhibit contrast between material properties, and that the theoretical upper bound can be reached by enlarging the asymmetry within the structure. 
Such results were obtained by applying heuristic optimization techniques.

Pernas-Salomón and Shmuel \cite{pernas2020symmetry} introduced --- by extending the approach of Willis --- a novel, supernatural property, that couples between the electric displacement and the velocity, and between the momentum and the electric field in piezoelectric composites. 
This coupling is now termed the electromomentum coupling, and it not only introduces new parameters to the design space of metamaterials, but also provides an additional degree of freedom than can be utilized to manipulate the wave propagation using non-mechanical stimuli. 
As extension to this work, Pernas-Salomón et al. \cite{pernas2021electromomentum} have shown that the electromomentum coupling generates additional asymmetry in the phase angle, an asymmetry that can be switched on and off by changing the electric circuit condition. 
This feature can be utilized to generate a phase difference in the reflection of waves.

Simply put, structural optimization assists the designer in defining the structural configuration, and seeks to determine the best assembly of materials, which is best suited to satisfy the constraint conditions for the objective in question.
In particular, topology optimization aims to determine the optimal material distribution in a given design space, and it is conceived as a class of structural optimization. 
Topology optimization has developed rapidly due to the advanced improvement in computational capabilities over the last decades \cite{christensen2008introduction, bendsoe1988generating, bendsoe1989optimal}.
One important class of applications of topology optimization is metamaterial design: material is optimally distributed in a periodic cell that represents the microstructure, such that metamaterial properties are obtained on the homogenized macro scale. 
This computational process is often termed inverse homogenization, and metamaterial properties such as negative Poisson's ratio and negative thermal expansion have been synthesized \cite{sigmund1994materials,sigmund1997design}, among many others.
Free Material Optimization (FMO) can be considered as an extension of topology optimization for the purpose of designing extremal materials. 
It was first introduced by Bends{\o}e et al. \cite{bendsoe1994analytical}, and later developed in \cite{zowe1997free}. 
The main goal of FMO is to determine the theoretical, ultimately best material properties and distribution in space, for a given objective \cite{kovcvara2008free}.
Using FMO, each constitutive property can vary independently of the other properties.
This removes all restrictions that would be imposed on metamaterial design if the composite was built from existing materials.
In the core of the current work, we employ inverse homogenization and FMO to maximize the electromomentum coupling.

The approach of Willis \cite{willis1981variational, willis1985nonlocal, willis1997dynamics} and Pernas-Salomón and Shmuel \cite{pernas2020symmetry} is based on Green's function of the relevant medium. 
The main drawbacks of this approach are that Green's function cannot be determined for most problems, and that it does not provide explicit expressions for the effective properties.
Hence, other methods are required. 
The Plane Wave Expansion (PWE) method was shown to be suitable for elastic, periodic problems. 
Here, similarly to the work of Muhafra et al. \cite{muhafra2021homogenization}, we adopt the same approach to obtain explicit expressions for the effective properties of one-dimensional, periodic piezoelectric composites that undergo waves of Bloch-Floquet type. 
In this approach we define the effective properties as the ensemble average of the microscopic fields, which is equivalent to volume averaging over the periodic part of the microscopic Bloch-Floquet waves. 
Moreover, our formulation of the governing equation we consider body forces, eigen-strain and volume charge. This formulation provides a unique set of effective properties.  

The main purpose of this study is to apply structural optimization techniques to maximize the electromomentum coupling in periodic, piezoelectric composites. 
The authors believe that the results will not only provide the optimal designs, but also establish guidelines on how to compose a laminate that maximizes the electromomentum coupling, using existing materials.
This can open new opportunities to manipulate the wave propagation and control the balance of momentum. 

The remainder of the paper is structured as follows: In Section \ref{chap:PWE} we introduce the one-dimensional homogenization scheme based on the PWE method. 
The first optimization formulation --- a discrete material choice --- is presented in Section \ref{sec:DMO}, followed by several gradient-based optimization problems presented in Section \ref{sec:GradientBased}, along with a detailed sensitivity analysis. 
In this Section we provide the theoretical upper bound of the electromomentum coupling, as a result of FMO.
The relation between the electromomentum coupling and specific structural and material properties is also investigated in Section \ref{sec:GradientBased}, allowing us to present the best applicable design. 
Finally, discussion of the method and concluding remarks are given in Section \ref{sec:sum}.










 




==> Prescribed.tex <==
%\chapter{Insights and reduced cases}
\label{Prescribed}














\pagebreak


==> properties.tex <==
\label{propmodel}
\subsection{The periodic medium}

Consider a periodic problem whose properties are periodic such that
\begin{equation}
\begin{array}{ccc}
\properties\left(\location+\sum_{j=1}^{m}n_{j}\unitv_{j}\right)=\properties\left(\location\right) & \textrm{for} & \properties=\stiffnesst,\B,\A,\density,\end{array}
\end{equation}
where $n_{j}\in\mathbb{Z}$, and the linear independent translation
vectors $\unitv_{j}\in\mathbb{R}^{m}$ define the unit cell $\unitv$.
We can expand the periodic functions in Fourier series, and identify
$\properties\left(\location\right)$ with a vector whose components
$\coeffgv{\properties}$ are the Fourier coefficients of $\properties\left(\location\right)$,
such that
\begin{equation}
\begin{array}{cc}
\coeffgv{\properties}=\left|\unitv\right|^{-1}\intop_{\unitv}\properties\left(\location\right)e^{-i\reciprocalvec\cdot\location}\mathrm{d\location}, & \properties\left(\location\right)=\sumGv\coeffgv{\properties}e^{i\reciprocalvec\cdot\location},\end{array}
\end{equation}
where $\reciprocalvec=\reciprocal_{i}\mathbf{e}_{i}=\frac{2\pi}{\unit{_{i}}}m^{(i)}\mathbf{e}_{i}$,
$m^{(i)}\in\mathbb{Z}$. We consider the presence of sources in the
form
\begin{equation}
\begin{array}{cc}
\sources\left(\location,t\right)=\sourcescon\mathrm{e}^{i\left(\wavevec\cdot\location-\angvel t\right)}, & \sources=\strainsot,\forcev,\charge,\end{array}
\end{equation}
where $\sourcescon$ is a constant. As a result, kinetic and the kinematic
fields are generated with the Bloch form 
\begin{equation}
\begin{aligned} & \begin{array}{cc}
\hfield\left(\location,t\right)=\periodic{\hfield}\left(\location\right)e^{i\left(\wavevec\cdot\location-\angvel t\right)}, & \hfield=\stresst,\elecdispv,\momentumv,\end{array}\\
 & \begin{array}{cc}
\wfield\left(\location,t\right)=\periodic{\wfield}\left(\location\right)e^{i\left(\wavevec\cdot\location-\angvel t\right)}, & \wfield=\dispv,\elecpot.\end{array}
\end{aligned}
\end{equation}
Note that $\periodic{\hfield}$ and $\periodic{\wfield}$ are periodic
with the same periodicity as the unit cell and the periodic parts
$\periodic{\hfield}\left(\location\right)$ and $\periodic{\wfield}\left(\location\right)$
can be expanded in Fourier series in the same manner that $\properties\left(\location\right)$
is expanded, such that
\begin{equation}
\periodic{\hfield}\left(\location\right)=\sumGv\coeffgv{\hfield}e^{i\reciprocalvec\cdot\location},\label{eq:FourierSeries}
\end{equation}
and the average over the single cell is defined by
\begin{equation}
\average{\hfield}=\left|\unitv\right|^{-1}\intop_{\unitv}\periodic{\hfield}\left(\location\right)\mathrm{d\location}.\label{eq:Four}
\end{equation}
We now define the effective fields by
\begin{equation}
\effective{\hfield}\left(\location,t\right)=\average{\hfield}e^{i\left(\wavevec\cdot\location-\angvel t\right)},\label{eq:EffectiveFields}
\end{equation}
where we keep in mind that $\sourcescon=\average{\sources}$ holds
trivially since $\sourcescon$ is a constant, and Eqs.~\eqref{eq:FourierSeries}-\eqref{eq:EffectiveFields}
hold for $\wfield$ in the same way.

\subsection{Derivation of the effective properties}
\label{sec:effect}
We begin by considering the Bloch form of Eq.~\eqref{eq:constPiezo},
namely,
\begin{equation}
\left(\begin{array}{c}
\periodic{\stress}\left(\locs\right)\\
\periodic{\elecdisp}\left(\locs\right)\\
\periodic{\momentum}\left(\locs\right)
\end{array}\right)e^{i\left(\wavenum\locs-\angvel t\right)}=\left(\begin{array}{ccc}
\stiffness\left(\locs\right) & \trans{\Bb}\left(\locs\right) & 0\\
\Bb\left(\locs\right) & -\Aa\left(\locs\right) & 0\\
0 & 0 & \density\left(\locs\right)
\end{array}\right)\left(\begin{array}{c}
\derivative{\periodic{\disp}\left(\locs\right)}+i\wavenum\periodic{\disp}\left(\locs\right)-\periodic{\strainso}\left(\locs\right)\\
\derivative{\periodic{\elecpot}\left(\locs\right)}+i\wavenum\periodic{\elecpot}\left(\locs\right)\\
-i\angvel\periodic{\disp}\left(\locs\right)
\end{array}\right)e^{i\left(\wavenum\locs-\angvel t\right)}.
\end{equation}
We expand the periodic parts of the fields and obtain
\begin{equation}
\left[\sumG\left(\begin{array}{c}
\coeffg{\stress}\\
\coeffg{\elecdisp}\\
\coeffg{\momentum}
\end{array}\right)e^{i\reciprocal x}-\sumGtG\left(\begin{array}{ccc}
\coeffg{\stiffness} & \trans{\coeffg{\Bb}} & 0\\
\coeffg{\Bb} & -\coeffg{\Aa} & 0\\
0 & 0 & \coeffg{\density}
\end{array}\right)\left(\begin{array}{c}
i\kGt\coeffgt{\disp}-\coeffgt{\eta}\\
i\kGt\coeffgt{\elecpot}\\
-i\angvel\coeffgt{\disp}
\end{array}\right)e^{i\left(\reciprocal+\reciprocalt\right)x}\right]e^{i\left(\wavenum\locs-\angvel t\right)}=0.\label{eq:ConstFourier}
\end{equation}
Since Eq.~\eqref{eq:ConstFourier} holds for any value of $\locs$
and $t$, the sums in the square brackets must vanish. We multiply
those sums by $e^{-i\reciprocal''x}$, and integrate the result over
the unit cell. Due to the orthogonality property of the Fourier series,
the only non-vanishing terms are those satisfying the condition $G''=\reciprocal+\reciprocalt$.
Thus, the resultant equation after changing $G''$ to $\reciprocal$
is
\begin{equation}
\left(\begin{array}{c}
\coeffg{\stress}\\
\coeffg{\elecdisp}\\
\coeffg{\momentum}
\end{array}\right)=\sumGt\left(\begin{array}{ccc}
\coeffggt{\stiffness} & \trans{\coeffggt{\Bb}} & 0\\
\coeffggt{\Bb} & -\coeffggt{\Aa} & 0\\
0 & 0 & \coeffggt{\density}
\end{array}\right)\left(\begin{array}{c}
i\kGt\coeffgt{\disp}-\coeffgt{\eta}\\
i\kGt\coeffgt{\elecpot}\\
-i\angvel\coeffgt{\disp}
\end{array}\right),\label{eq:Piezo-cosntFT}
\end{equation}
where $\ggt{\left(\circ\right)}G{G'}$ denotes the Fourier coefficient
of $\left(\circ\right)$ along the basis function $e^{i\left(\reciprocal-\reciprocalt\right)x}$
. In the same manner, Eq.~\eqref{eq:PiezoGov} reads 
\begin{equation}
\begin{aligned} & \left(\derivative{\periodic{\stress}}+i\wavenum\periodic{\stress}+\periodic{\force}\right)e^{i\left(\wavenum\locs-\angvel t\right)}=-i\angvel\periodic{\momentum}e^{i\left(\wavenum\locs-\angvel t\right)},\\
 & \left(\derivative{\periodic{\elecdisp}}+i\wavenum\periodic{\elecdisp}\right)e^{i\left(\wavenum\locs-\angvel t\right)}=\periodic{\charge}e^{i\left(\wavenum\locs-\angvel t\right)}.
\end{aligned}
\end{equation}
Once again, we expand the periodic parts to 
\begin{equation}
\begin{aligned} & \sumG\left[i\kG\coeffg{\stress}+\coeffg{\force}\right]e^{i\reciprocal x}e^{i\left(\wavenum\locs-\angvel t\right)}=-i\angvel\sumG\coeffg{\momentum}e^{i\reciprocal x}e^{i\left(\wavenum\locs-\angvel t\right)},\\
 & \sumG\left[i\kG\coeffg{\elecdisp}\right]e^{i\reciprocal x}e^{i\left(\wavenum\locs-\angvel t\right)}=\sumG\coeffg{\charge}e^{i\reciprocal x}e^{i\left(\wavenum\locs-\angvel t\right)}.
\end{aligned}
\end{equation}
A truncation to a finite number of plane waves $\numwaves$ is carried
out for implementational purposes, say by $-s\le m\le s$, such that
$\numwaves=2s+1$. We multiply those sums by $e^{-i\reciprocal''x}$,
and integrate the result over the unit-cell. Due to the orthogonality
property of the Fourier series, the only non-vanishing terms are those
satisfying the condition $G''=\reciprocal$. We can write for any
$\reciprocal$ 
\begin{equation}
\g{\opgov}^{\mathsf{T}}\g{\kineticv}=-\g{\forces},\label{eq:govG}
\end{equation}
where
\begin{equation}
\g{\opgov}=\left(\begin{array}{cc}
i\kG & 0\\
0 & i\kG\\
i\angvel & 0
\end{array}\right),\g{\kineticv}=\left(\begin{array}{c}
\coeffg{\stress}\\
\coeffg{\elecdisp}\\
\coeffg{\momentum}
\end{array}\right),\g{\forces}=\left(\begin{array}{c}
\coeffg{\force}\\
-\coeffg{\charge}
\end{array}\right).
\end{equation}
Next, we assemble all the matrix equations associated with Eq.~\eqref{eq:govG}
for each $\reciprocal$, to a single matrix system in the form
\begin{equation}
\trans{\assembly{\opgov}}\assembly{\kineticv}=-\assembly{\forces},\label{eq:GovCona}
\end{equation}
where $\assembly{\forces}$ is a column vector of $2\numwaves$ components,
which contains all the Fourier coefficients of $\coeffg{\force}$
and $\coeffg{\charge}$, $\assembly{\kineticv}$ is a column vector
of $3\numwaves$ components, which contains all the Fourier coefficients
of $\coeffg{\stress},\coeffg{\elecdisp}$ and $\coeffg{\momentum}$,
and $\assembly{\opgov}$ is a $3\numwaves\times2\numwaves$ matrix
whose components are given in the Appendix. Note that $\assembly{\kineticv}$
is obtained in the manner by assembling the matrix equations associated
with Eq.~\eqref{eq:Piezo-cosntFT}, such that
\begin{equation}
\assembly{\kineticv}=\assembly{\prop}\left(\assembly{\opcon}\assembly{\kinematicv}-\assembly{\strainsov}\right)\label{eq:GovConb}
\end{equation}
where $\assembly{\prop}$ is a $3\numwaves\times3\numwaves$ matrix
that assembles the Fourier components of the mechanical properties,
$\assembly{\opcon}$ is a $3\numwaves\times2\numwaves$ matrix that
assembles the Fourier components of the differential operators, $\assembly{\kinematicv}$
is a column vector of $2\numwaves$ components that assembles the
Fourier components of the displacement and the electric potential
and $\assembly{\strainsov}$ is a column vector of $3\numwaves$ components
that assembles the Fourier components of the inelastic strain. Explicit
expressions for Eqs.~\eqref{eq:GovCona} and \eqref{eq:GovConb}
are given in the Appendix. We now extract from Eq.~\eqref{eq:GovConb}
the average fields out of $\assembly{\kineticv}$, and write them
as

\begin{equation}
\average{\kineticv}\coloneqq\left(\begin{array}{c}
\average{\stress}\\
\average{\elecdisp}\\
\average{\momentum}
\end{array}\right)\equiv\left(\begin{array}{c}
\coeffz{\stress}\\
\coeffz{\elecdisp}\\
\coeffz{\momentum}
\end{array}\right)=\zero{\prop}\left\{ \zero{\opcon}\average{\kinematicv}-\average{\strainsov}\right\} +\reduced{\prop}\reduced{\opcon}\reduced{\kinematicv},\label{eq:constEFF}
\end{equation}
where $\zero{\opcon}$ and $\zero{\prop}$ are the parts of the matrices
that multiply the average fields (associated with $\reciprocal=0$)
and $\reduced{\left(\circ\right)}$ denotes the reduced matrix or
vector without the $\reciprocal=0$ terms\footnote{Here $\zero{\prop}$ is a $3\times3$ matrix, $\zero{\opcon}$ is
a $3\times2$ matrix, $\average{\kinematicv}$ is a vector with 2
components, $\average{\strainsov}$ is a vector with 3 components,
$\reduced{\prop}$ is a $3\times\left(3\numwaves-3\right)$ matrix,
$\reduced{\opcon}$ is a $\left(3\numwaves-3\right)\times\left(2\numwaves-2\right)$
matrix and $\reduced{\kinematicv}$ is a vector with $2\numwaves$
components.}. Our goal is to express the terms $\reduced{\kinematicv}$ using
$\average{\kinematicv}$ and $\average{\strainsov}$. To this end,
we first write Eq.~\eqref{eq:GovCona} in the form Ren� Pernas-Salom�n
\begin{equation}
\assembly{\trans{\opgov}}\assembly{\prop}\left(\assembly{\opcon}\assembly{\kinematicv}-\assembly{\strainsov}\right)=-\assembly{\forces}.\label{eq:ExpandGOV}
\end{equation}
Next, we utilize the equations that do not include $\reciprocal=0$
in Eq.~\eqref{eq:ExpandGOV} to write
\begin{equation}
\reduced{\Q}\reduced{\kinematicv}=-\DL\left\{ \zero{\opcon}\average{\kinematicv}-\average{\strainsov}\right\} ,\label{eq:PiezoGovGne0}
\end{equation}
where $\reduced{\Q}$ is a square matrix which contain the terms which
do not multiply the average fields, and $\DL$ is the part of the
matrix $\trans{\opgov}\prop$ which multiplies the average fields.
This process is similar to the one carried out in (cite Rene's paper).
We are now able to express the fluctuating terms of $\kinematicv$
using its average value and the properties of the composite, namely,
\begin{equation}
\reduced{\kinematicv}=-\reduced{\Q}^{-1}\DL\left\{ \zero{\opcon}\average{\kinematicv}-\average{\strainsov}\right\} .\label{eq:PsiNeZero}
\end{equation}
Accordingly, Eq.~\eqref{eq:constEFF} reads

\begin{equation}
\average{\kineticv}=\zero{\prop}\left\{ \zero{\opcon}\average{\kinematicv}-\average{\strainsov}\right\} -\reduced{\prop}\reduced{\opcon}\reduced{\Q}^{-1}\DL\left\{ \zero{\opcon}\average{\kinematicv}-\average{\strainsov}\right\} .\label{eq:Compare}
\end{equation}
We can identify the effective properties in Eq.~\eqref{eq:Compare}
by comparing them with the generalized Willis relations given by Eq.~\eqref{eq:GenWillis},
\emph{i.e.},
\begin{equation}
\average{\kineticv}=\left(\begin{array}{ccc}
\effectiveprop{\stiffness} & \dag{\effectiveprop{\Bb}} & \effectiveprop{\coupling}\\
\effectiveprop{\Bb} & -\effectiveprop{\Aa} & \effectiveprop{\couplingele}\\
\dag{\effectiveprop{\coupling}} & \dag{\effectiveprop{\couplingele}} & \effectiveprop{\density}
\end{array}\right)\left\{ \zero{\opcon}\average{\kinematicv}-\average{\strainsov}\right\} ,
\end{equation}
such that
\begin{equation}
\underline{W}=\left(\begin{array}{ccc}
\effectiveprop{\stiffness} & \trans{\effectiveprop{\Bb}} & \effectiveprop{\coupling}\\
\effectiveprop{\Bb} & -\effectiveprop{\Aa} & \effectiveprop{\couplingele}\\
\dag{\effectiveprop{\coupling}} & \dag{\effectiveprop{\couplingele}} & \effectiveprop{\density}
\end{array}\right)=\zero{\prop}-\reduced{\prop}\reduced{\opcon}\reduced{\Q}^{-1}\DL.\label{eq:W}
\end{equation}

